Forecasting infectious disease prevalence with associated uncertainty using neural networks

Infectious diseases pose significant human and economic burdens. Accurately forecasting disease incidence can enable public health agencies to respond effectively to existing or emerging diseases. Despite progress in the field, developing accurate forecasting models remains a significant challenge. This thesis proposes two methodological frameworks using neural networks (NNs) with associated uncertainty estimates - a critical component limiting the application of NNs to epidemic forecasting thus far. We develop our frameworks by forecasting influenza-like illness (ILI) in the United States. Our first proposed method uses Web search activity data in conjunction with historical ILI rates as observations for training NN architectures. Our models incorporate Bayesian layers to produce uncertainty intervals, positioning themselves as legitimate alternatives to more conventional approaches. The best performing architecture: iterative recurrent neural network (IRNN), reduces mean absolute error by 10.3% and improves Skill by 17.1% on average in forecasting tasks across four flu seasons compared to the state-of-the-art. We build on this method by introducing IRNNs, an architecture which changes the sampling procedure in the IRNN to improve the uncertainty estimation. Our second framework uses neural ordinary differential equations to bridge the gap between mechanistic compartmental models and NNs; benefiting from the physical constraints that compartmental models provide. We evaluate eight neural ODE models utilising a mixture of ILI rates and Web search activity data to provide forecasts. These are compared with the IRNN and IRNN0 - the IRNN using only ILI rates. Models trained without Web search activity data outperform the IRNN0 by 16% in terms of Skill. Future work should focus on more effectively using neural ODEs with Web search data to compete with the best performing IRNN.

==> Tables/Chapter_1/table-performance-NNs.tex <==


\begin{tabular}{p{0.3cm}p{0.8cm} P{0.8cm}P{0.8cm}P{0.7cm} P{0.8cm}P{0.8cm}P{0.7cm} P{0.8cm}P{0.8cm}P{0.7cm} P{0.8cm}P{0.8cm}P{0.7cm} P{0.8cm}P{0.8cm}P{0.7cm}}
 & &\multicolumn{3}{c}{2015/16} & \multicolumn{3}{c}{2016/17} & \multicolumn{3}{c}{2017/18} & \multicolumn{3}{c}{2018/19} & \multicolumn{3}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
$\gamma$ & & IRNN & SRNN & FF & IRNN & SRNN & FF & IRNN & SRN & FF & IRNN & SRNN & FF & IRNN & SRNN & FF\\
\midrule
7    &    NLL       &            0.20 &       \bf{-0.38} &           -0.19 &            0.38 &       \bf{-0.29} &           -0.06 &               0.65 &       \bf{0.07} &            0.52 &            0.32 &       \bf{-0.49} &            0.12 &            0.39 &       \bf{-0.27} &            0.10 \\
     &   CRPS       &            0.18 &        \bf{0.09} &            0.10 &            0.24 &        \bf{0.12} &            0.14 &               0.31 &       \bf{0.17} &            0.33 &            0.21 &        \bf{0.08} &            0.19 &            0.23 &        \bf{0.12} &            0.19 \\
     &  Skill       &            0.73 &        \bf{0.95} &            0.89 &            0.59 &        \bf{0.85} &            0.78 &               0.49 &       \bf{0.77} &            0.54 &            0.62 &        \bf{0.95} &            0.70 &            0.60 &        \bf{0.87} &            0.72 \\
     &    MAE       &            0.26 &        \bf{0.13} &            0.13 &            0.33 &        \bf{0.18} &            0.20 &               0.37 &       \bf{0.25} &            0.49 &            0.28 &        \bf{0.11} &            0.27 &            0.31 &        \bf{0.17} &            0.27 \\
     &   $r$        &            0.85 &        \bf{0.97} &            0.97 &            0.92 &        \bf{0.99} &            0.99 &               0.98 &       \bf{0.99} &            0.98 &            0.93 &        \bf{0.99} &            0.97 &            0.92 &        \bf{0.98} &            0.98 \\
     % & \CalibMetric &       \bf{0.04} &             0.10 &            0.16 &            0.03 &        \bf{0.02} &            0.10 &               0.09 &            0.04 &       \bf{0.03} &            0.13 &             0.10 &       \bf{0.03} &       \bf{0.05} &             0.09 &            0.08 \\
\midrule
14   &    NLL       &       \bf{0.18} &             0.35 &            0.49 &       \bf{0.36} &             0.53 &            0.46 &          \bf{0.64} &            3.28 &            0.94 &            0.30 &       \bf{0.27} &             0.64 &       \bf{0.37} &             1.11 &            0.63 \\
     &   CRPS       &       \bf{0.18} &             0.21 &            0.20 &            0.24 &             0.27 &       \bf{0.19} &          \bf{0.31} &            0.72 &            0.39 &       \bf{0.21} &             0.21 &            0.27 &       \bf{0.24} &             0.35 &            0.26 \\
     &  Skill       &       \bf{0.73} &             0.69 &            0.61 &       \bf{0.59} &             0.54 &            0.59 &          \bf{0.49} &            0.11 &            0.39 &            0.63 &        \bf{0.67} &            0.52 &       \bf{0.60} &             0.40 &            0.52 \\
     &    MAE       &            0.26 &             0.29 &       \bf{0.25} &            0.33 &             0.36 &       \bf{0.22} &          \bf{0.38} &            0.88 &            0.50 &       \bf{0.28} &             0.29 &            0.40 &       \bf{0.31} &             0.45 &            0.34 \\
     &   $r$        &            0.85 &             0.85 &       \bf{0.91} &            0.92 &             0.92 &       \bf{0.97} &          \bf{0.98} &            0.88 &            0.94 &            0.93 &        \bf{0.94} &            0.91 &            0.92 &             0.90 &       \bf{0.93} \\
     % & \CalibMetric &       \bf{0.02} &             0.03 &            0.18 &       \bf{0.04} &             0.05 &            0.23 &          \bf{0.08} &            0.20 &            0.17 &            0.12 &        \bf{0.04} &            0.07 &       \bf{0.08} &             0.11 &            0.15 \\
\midrule
21   &    NLL       &       \bf{0.32} &             0.85 &            0.85 &       \bf{0.63} &             0.80 &            0.88 &          \bf{0.78} &            2.08 &            1.50 &       \bf{0.47} &             0.88 &            1.06 &       \bf{0.55} &             1.15 &            1.07 \\
     &   CRPS       &       \bf{0.23} &             0.33 &            0.28 &            0.31 &        \bf{0.29} &            0.30 &          \bf{0.42} &            0.70 &            0.61 &       \bf{0.27} &             0.33 &            0.38 &       \bf{0.30} &             0.41 &            0.39 \\
     &  Skill       &       \bf{0.65} &             0.51 &            0.45 &       \bf{0.49} &             0.46 &            0.42 &          \bf{0.43} &            0.15 &            0.24 &       \bf{0.56} &             0.45 &            0.37 &       \bf{0.52} &             0.36 &            0.36 \\
     &    MAE       &       \bf{0.32} &             0.45 &            0.36 &            0.42 &             0.39 &       \bf{0.35} &          \bf{0.56} &            0.90 &            0.79 &       \bf{0.37} &             0.46 &            0.53 &       \bf{0.42} &             0.55 &            0.51 \\
     &   $r$        &       \bf{0.81} &             0.68 &            0.77 &            0.85 &             0.89 &       \bf{0.93} &          \bf{0.94} &            0.89 &            0.86 &       \bf{0.88} &             0.85 &            0.84 &       \bf{0.87} &             0.83 &            0.85 \\
     % & \CalibMetric &       \bf{0.02} &             0.10 &            0.18 &       \bf{0.03} &             0.03 &            0.22 &          \bf{0.04} &            0.15 &            0.16 &            0.07 &        \bf{0.06} &            0.13 &       \bf{0.08} &             0.11 &            0.15 \\
\midrule
28   &    NLL       &       \bf{0.53} &             1.07 &            1.07 &       \bf{0.73} &             1.19 &            1.09 &          \bf{1.32} &            3.82 &            1.80 &       \bf{0.54} &             0.98 &            1.27 &       \bf{0.78} &             1.76 &            1.31 \\
     &   CRPS       &       \bf{0.31} &             0.40 &            0.35 &       \bf{0.35} &             0.35 &            0.38 &          \bf{0.57} &            0.88 &            0.80 &       \bf{0.30} &             0.36 &            0.46 &       \bf{0.38} &             0.50 &            0.50 \\
     &  Skill       &       \bf{0.54} &             0.41 &            0.36 &       \bf{0.45} &             0.34 &            0.35 &          \bf{0.27} &            0.06 &            0.18 &       \bf{0.53} &             0.40 &            0.30 &       \bf{0.43} &             0.24 &            0.29 \\
     &    MAE       &            0.45 &             0.56 &       \bf{0.40} &            0.49 &             0.44 &       \bf{0.41} &          \bf{0.73} &            1.05 &            1.07 &       \bf{0.43} &             0.49 &            0.63 &       \bf{0.53} &             0.64 &            0.63 \\
     &   $r$        &       \bf{0.80} &             0.55 &            0.60 &            0.81 &             0.89 &       \bf{0.92} &          \bf{0.91} &            0.84 &            0.76 &            0.85 &        \bf{0.86} &            0.77 &       \bf{0.84} &             0.78 &            0.76 \\
     % & \CalibMetric &       \bf{0.05} &             0.11 &            0.22 &       \bf{0.04} &             0.06 &            0.25 &          \bf{0.07} &            0.13 &            0.12 &       \bf{0.04} &             0.05 &            0.13 &       \bf{0.07} &             0.12 &            0.15 \\
\bottomrule
\end{tabular}


% \midrule
% 7    &    NLL &            0.15 &       \bf{-0.43} &           -0.21 &            0.32 &       \bf{-0.31} &           -0.09 &            0.58 &       \bf{-0.01} &            0.46 &            0.28 &       \bf{-0.45} &            0.10 &            0.33 &       \bf{-0.30} &            0.06 \\
%      &   CRPS &            0.18 &        \bf{0.09} &            0.10 &            0.23 &        \bf{0.12} &            0.13 &            0.30 &        \bf{0.16} &            0.32 &            0.20 &        \bf{0.08} &            0.18 &            0.23 &        \bf{0.11} &            0.18 \\
%      &  Skill &            0.74 &        \bf{0.96} &            0.90 &            0.60 &        \bf{0.87} &            0.79 &            0.51 &        \bf{0.79} &            0.55 &            0.64 &        \bf{0.95} &            0.71 &            0.62 &        \bf{0.89} &            0.73 \\
%      &    MAE &            0.25 &        \bf{0.12} &            0.12 &            0.32 &        \bf{0.17} &            0.19 &            0.36 &        \bf{0.23} &            0.47 &            0.28 &        \bf{0.12} &            0.27 &            0.30 &        \bf{0.16} &            0.26 \\
%      &   $r$  &            0.86 &        \bf{0.97} &            0.97 &            0.93 &             0.99 &       \bf{0.99} &            0.98 &        \bf{0.99} &            0.98 &            0.94 &        \bf{0.99} &            0.97 &            0.93 &        \bf{0.99} &            0.98 \\
%      &    \CalibMetric &   0.03 &        \bf{0.11} &            0.17 &       \bf{0.05} &             0.01 &            0.10 &       \bf{0.09} &             0.03 &            0.02 &            0.12 &             0.07 &       \bf{0.02} &       \bf{0.05} &             0.09 &            0.08 \\
% \midrule
% 14   &    NLL &       \bf{0.13} &             0.29 &            0.46 &       \bf{0.30} &             0.43 &            0.42 &       \bf{0.57} &             2.90 &            0.89 &            0.27 &        \bf{0.20} &            0.60 &       \bf{0.32} &             0.95 &            0.59 \\
%      &   CRPS &       \bf{0.18} &             0.19 &            0.19 &            0.23 &             0.25 &       \bf{0.19} &       \bf{0.30} &             0.65 &            0.38 &            0.20 &        \bf{0.19} &            0.27 &       \bf{0.23} &             0.32 &            0.25 \\
%      &  Skill &       \bf{0.74} &             0.71 &            0.62 &            0.60 &             0.58 &       \bf{0.61} &       \bf{0.50} &             0.14 &            0.41 &            0.64 &        \bf{0.70} &            0.53 &       \bf{0.61} &             0.45 &            0.53 \\
%      &    MAE &            0.25 &             0.27 &       \bf{0.24} &            0.32 &             0.33 &       \bf{0.21} &       \bf{0.37} &             0.80 &            0.49 &            0.28 &        \bf{0.27} &            0.39 &       \bf{0.30} &             0.42 &            0.33 \\
%      &   $r$  &            0.87 &             0.88 &       \bf{0.92} &            0.93 &             0.93 &       \bf{0.97} &       \bf{0.98} &             0.89 &            0.95 &            0.94 &        \bf{0.95} &            0.91 &            0.93 &             0.91 &       \bf{0.94} \\
%      &    \CalibMetric &   0.03 &        \bf{0.03} &            0.19 &       \bf{0.05} &             0.04 &            0.24 &            0.08 &             0.19 &       \bf{0.18} &       \bf{0.11} &             0.05 &            0.07 &       \bf{0.08} &             0.11 &            0.15 \\
% \midrule
% 21   &    NLL &       \bf{0.26} &             0.73 &            0.83 &       \bf{0.56} &             0.71 &            0.85 &       \bf{0.70} &             1.87 &            1.45 &       \bf{0.42} &             0.80 &            1.02 &       \bf{0.48} &             1.03 &            1.04 \\
%      &   CRPS &       \bf{0.22} &             0.30 &            0.28 &            0.29 &        \bf{0.28} &            0.29 &       \bf{0.40} &             0.64 &            0.59 &       \bf{0.26} &             0.31 &            0.37 &       \bf{0.29} &             0.38 &            0.38 \\
%      &  Skill &       \bf{0.66} &             0.54 &            0.46 &            0.50 &        \bf{0.50} &            0.43 &       \bf{0.45} &             0.19 &            0.25 &       \bf{0.57} &             0.48 &            0.38 &       \bf{0.54} &             0.39 &            0.37 \\
%      &    MAE &       \bf{0.30} &             0.42 &            0.35 &            0.40 &             0.37 &       \bf{0.34} &       \bf{0.54} &             0.83 &            0.77 &       \bf{0.36} &             0.44 &            0.51 &       \bf{0.40} &             0.52 &            0.49 \\
%      &    $r$ &       \bf{0.83} &             0.73 &            0.80 &            0.87 &             0.91 &       \bf{0.94} &       \bf{0.94} &             0.90 &            0.87 &       \bf{0.89} &             0.87 &            0.85 &       \bf{0.88} &             0.85 &            0.86 \\
%      &    \CalibMetric&\bf{0.02}&             0.08 &            0.19 &       \bf{0.03} &             0.03 &            0.23 &            0.04 &             0.15 &       \bf{0.16} &            0.07 &        \bf{0.06} &            0.14 &       \bf{0.08} &             0.11 &            0.15 \\
% \midrule
% 28   &    NLL &       \bf{0.47} &             0.95 &            1.04 &       \bf{0.68} &             1.03 &            1.06 &       \bf{1.23} &             3.36 &            1.75 &       \bf{0.48} &             0.85 &            1.23 &       \bf{0.71} &             1.55 &            1.27 \\
%      &   CRPS &       \bf{0.30} &             0.37 &            0.34 &            0.34 &        \bf{0.32} &            0.37 &       \bf{0.55} &             0.79 &            0.77 &            0.29 &        \bf{0.33} &            0.45 &       \bf{0.37} &             0.45 &            0.48 \\
%      &  Skill &       \bf{0.55} &             0.44 &            0.37 &       \bf{0.46} &             0.38 &            0.36 &       \bf{0.29} &             0.09 &            0.19 &       \bf{0.55} &             0.44 &            0.31 &       \bf{0.45} &             0.28 &            0.30 \\
%      &    MAE &            0.44 &             0.51 &       \bf{0.38} &            0.47 &        \bf{0.40} &            0.40 &       \bf{0.70} &             0.94 &            1.04 &            0.42 &        \bf{0.44} &            0.61 &       \bf{0.51} &             0.57 &            0.61 \\
%      &   $r$ &       \bf{0.82}  &             0.60 &            0.65 &            0.82 &             0.90 &       \bf{0.93} &       \bf{0.92} &             0.85 &            0.77 &            0.87 &        \bf{0.88} &            0.79 &       \bf{0.86} &             0.81 &            0.79 \\
%      &    \CalibMetric&\bf{0.05}&             0.08 &            0.23 &            0.05 &        \bf{0.10} &            0.25 &       \bf{0.07} &             0.08 &            0.12 &       \bf{0.04} &             0.04 &            0.13 &       \bf{0.07} &             0.12 &            0.15 \\
% \bottomrule


==> Tables/Chapter_1/table-performance-dante-ElN.tex <==


% \begin{tabular}{p{1.1cm} p{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} | P{0.8cm} P{0.8cm}}

\begin{tabular}{p{1.1cm} p{1.1cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} | P{0.87cm} P{0.87cm} P{0.7cm}}
Horizon & Metric  &\multicolumn{2}{c}{2015/16} & \multicolumn{2}{c}{2016/17} & \multicolumn{2}{c}{2017/18} & \multicolumn{2}{c}{2018/19} & \multicolumn{5}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-15}
$\gamma$  & & Dante & NN & Dante & NN & Dante & NN & Dante & NN & Dante & NN & Eln & NN$_a$ & NN$_b$\\
\midrule
7   & Skill         & 0.67      & \bf{0.75} & \bf{0.63} & 0.53      & 0.45      & \bf{0.53} & \bf{0.62} & 0.61      & 0.59      &\bf{0.60}  &       & 0.85  & 0.88\\
    & MAE           & \bf{0.22} & 0.26      & \bf{0.19} & 0.35      & 0.39      & \bf{0.38} & \bf{0.21} & 0.28      & \bf{0.25} & 0.32      & 0.18  & 0.18  & 0.17\\
    & $r$           & \bf{0.88} & 0.81      & \bf{0.96} & 0.91      & 0.97      & \bf{0.98} & \bf{0.97} & 0.90      & \bf{0.94} & 0.90      & 0.98  & 0.98  & 0.98\\
    % & \CalibMetric  & 0.09      & \bf{0.03} & 0.18      & \bf{0.05} & \bf{0.09} & 0.04      & 0.16      & \bf{0.15} & 0.13      & \bf{0.07} & 0.09  & 0.08\\
\midrule
14  & Skill         & 0.54      & \bf{0.74} & \bf{0.54} & 0.53      & 0.29      & \bf{0.53} & 0.52      & \bf{0.61} & 0.46      & \bf{0.59} &       & 0.55  & 0.59\\
    & MAE           & 0.38      & \bf{0.28} & \bf{0.32} & 0.35      & 0.64      & \bf{0.39} & 0.33      & \bf{0.28} & 0.42      & \bf{0.33} & 0.35  & 0.35  & 0.34\\
    & $r$           & 0.64      & \bf{0.79} & 0.91      & \bf{0.91} & 0.90      & \bf{0.98} & \bf{0.92} & 0.90      & 0.84      & \bf{0.89} & 0.91  & 0.89  & 0.89\\
    % & \CalibMetric  & \bf{0.05} & 0.06      & 0.10      & \bf{0.04} & \bf{0.04} & 0.04      & \bf{0.10} & 0.16      & \bf{0.07} & 0.08      & 0.07  & 0.06\\
\midrule
21  & Skill         & 0.44      & \bf{0.64} & \bf{0.48} & 0.43      & 0.21      & \bf{0.30} & 0.46      & \bf{0.52} & 0.38      & \bf{0.45} &       & 0.47  & 0.48\\
    & MAE           & 0.48      & \bf{0.37} & \bf{0.38} & 0.45      & 0.86      & \bf{0.62} & \bf{0.40} & 0.44      & 0.53      & \bf{0.47} & 0.62  & 0.48  & 0.46\\
    & $r$           & 0.36      & \bf{0.67} & \bf{0.87} & 0.83      & 0.82      & \bf{0.94} & \bf{0.89} & 0.82      & 0.73      & \bf{0.81} & 0.71  & 0.81  & 0.81\\
    % & \CalibMetric  & \bf{0.06} & 0.09      & 0.07      & \bf{0.11} & \bf{0.03} & 0.10      & \bf{0.10} & 0.04      & \bf{0.07} & 0.09      & 0.07  & 0.07\\
\midrule
28  & Skill         & 0.37      & \bf{0.53} & \bf{0.46} & 0.38      & \bf{0.17} & 0.14      & 0.42      & \bf{0.45} & 0.33      & \bf{0.33} &       & 0.37  & 0.40\\
    & MAE           & 0.54      & \bf{0.47} & \bf{0.39} & 0.50      & 1.06      & \bf{0.85} & \bf{0.45} & 0.58      & 0.61      & \bf{0.60} & 0.80  & 0.61  & 0.58\\
    & $r$           & 0.23      & \bf{0.63} & \bf{0.88} & 0.79      & 0.76      & \bf{0.92} & \bf{0.86} & 0.79      & 0.68      & \bf{0.78} & 0.58  & 0.78  & 0.79\\
    % & \CalibMetric  & \bf{0.05} & 0.12      & \bf{0.08} & 0.13      & \bf{0.08} & 0.22      & 0.10      & \bf{0.03} & \bf{0.08} & 0.12      & 0.08  & 0.10\\
\bottomrule
\end{tabular}


==> Tables/Chapter_1/table-performance-dante.tex <==


% \begin{tabular}{p{1.1cm} p{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} P{1.1cm} | P{0.8cm} P{0.8cm}}

\begin{tabular}{p{1.1cm} p{1.1cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} P{0.7cm} | P{0.87cm} P{0.7cm}}
Horizon & Metric  &\multicolumn{2}{c}{2015/16} & \multicolumn{2}{c}{2016/17} & \multicolumn{2}{c}{2017/18} & \multicolumn{2}{c}{2018/19} & \multicolumn{4}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-14}
$\gamma$  & & Dante & NN & Dante & NN & Dante & NN & Dante & NN & Dante & NN & NN$_a$ & NN$_b$\\
\midrule
7   & Skill         & 0.67      & \bf{0.75} & \bf{0.63} & 0.53      & 0.45      & \bf{0.53} & \bf{0.62} & 0.61      & 0.59      &\bf{0.60}  & 0.85  & 0.88\\
    & MAE           & \bf{0.22} & 0.26      & \bf{0.19} & 0.35      & 0.39      & \bf{0.38} & \bf{0.21} & 0.28      & \bf{0.25} & 0.32      & 0.18  & 0.17\\
    & $r$           & \bf{0.88} & 0.81      & \bf{0.96} & 0.91      & 0.97      & \bf{0.98} & \bf{0.97} & 0.90      & \bf{0.94} & 0.90      & 0.98  & 0.98\\
    % & \CalibMetric  & 0.09      & \bf{0.03} & 0.18      & \bf{0.05} & \bf{0.09} & 0.04      & 0.16      & \bf{0.15} & 0.13      & \bf{0.07} & 0.09  & 0.08\\
\midrule
14  & Skill         & 0.54      & \bf{0.74} & \bf{0.54} & 0.53      & 0.29      & \bf{0.53} & 0.52      & \bf{0.61} & 0.46      & \bf{0.59} & 0.55  & 0.59\\
    & MAE           & 0.38      & \bf{0.28} & \bf{0.32} & 0.35      & 0.64      & \bf{0.39} & 0.33      & \bf{0.28} & 0.42      & \bf{0.33} & 0.35  & 0.34\\
    & $r$           & 0.64      & \bf{0.79} & 0.91      & \bf{0.91} & 0.90      & \bf{0.98} & \bf{0.92} & 0.90      & 0.84      & \bf{0.89} & 0.89  & 0.89\\
    % & \CalibMetric  & \bf{0.05} & 0.06      & 0.10      & \bf{0.04} & \bf{0.04} & 0.04      & \bf{0.10} & 0.16      & \bf{0.07} & 0.08      & 0.07  & 0.06\\
\midrule
21  & Skill         & 0.44      & \bf{0.64} & \bf{0.48} & 0.43      & 0.21      & \bf{0.30} & 0.46      & \bf{0.52} & 0.38      & \bf{0.45} & 0.47  & 0.48\\
    & MAE           & 0.48      & \bf{0.37} & \bf{0.38} & 0.45      & 0.86      & \bf{0.62} & \bf{0.40} & 0.44      & 0.53      & \bf{0.47} & 0.48  & 0.46\\
    & $r$           & 0.36      & \bf{0.67} & \bf{0.87} & 0.83      & 0.82      & \bf{0.94} & \bf{0.89} & 0.82      & 0.73      & \bf{0.81} & 0.81  & 0.81\\
    % & \CalibMetric  & \bf{0.06} & 0.09      & 0.07      & \bf{0.11} & \bf{0.03} & 0.10      & \bf{0.10} & 0.04      & \bf{0.07} & 0.09      & 0.07  & 0.07\\
\midrule
28  & Skill         & 0.37      & \bf{0.53} & \bf{0.46} & 0.38      & \bf{0.17} & 0.14      & 0.42      & \bf{0.45} & 0.33      & \bf{0.33} & 0.37  & 0.40\\
    & MAE           & 0.54      & \bf{0.47} & \bf{0.39} & 0.50      & 1.06      & \bf{0.85} & \bf{0.45} & 0.58      & 0.61      & \bf{0.60} & 0.61  & 0.58\\
    & $r$           & 0.23      & \bf{0.63} & \bf{0.88} & 0.79      & 0.76      & \bf{0.92} & \bf{0.86} & 0.79      & 0.68      & \bf{0.78} & 0.78  & 0.79\\
    % & \CalibMetric  & \bf{0.05} & 0.12      & \bf{0.08} & 0.13      & \bf{0.08} & 0.22      & 0.10      & \bf{0.03} & \bf{0.08} & 0.12      & 0.08  & 0.10\\
\bottomrule
\end{tabular}


==> Tables/Chapter_1/table-performance-meta-dante.tex <==
\begin{tabular}{l ccc}
\toprule
Horizon
        & \multicolumn{3}{c}{$\gamma = 21$} \\
\toprule
Metric
        & Dante     & NN        & NN$_b$ \\
\midrule
$\delta$-p (days)          &
        \textbf{-70}, 14, 14, 14 & -49, 14, -14, -35     & -49, 14, -28, -35  \\
Avg. $\delta$-$y_{\text{p}}$ &
        0.99        & 0.70      & 0.59      \\
MAE-p               &
        0.84        & 0.75      & 0.76      \\
SMAPE-p (\%)        &
        20.19       & 15.57     & 15.69     \\
\bottomrule
\\
\\
\toprule
Horizon & \multicolumn{3}{c}{$\gamma = 28$} \\
\toprule
Metric
        & Dante     & NN        & NN$_b$ \\
\midrule
$\delta$-p (days)          &
        \textbf{-70}, 14, 7, 14  & -42, -21, -21, -28    & -42, -21, -21, -28 \\

Avg. $\delta$-$y_{\text{p}}$ &
        0.67        & 1.01      & 0.87      \\
MAE-p               &
        1.09        & 0.89      & 0.88      \\
SMAPE-p (\%)        &
        \textbf{26.24}       & 17.72     & 17.57     \\

\bottomrule
\end{tabular}




==> Tables/Chapter_2/IRNN_Comparison.tex <==
\begin{tabular}{p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}p{1.1cm}}
\ Horizon & Metric  &\multicolumn{3}{c}{2015/16} & \multicolumn{3}{c}{2016/17} & \multicolumn{3}{c}{2017/18} & \multicolumn{3}{c}{2018/19} & \multicolumn{3}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
$\gamma$   &     &            IRNN &         \SEIRNN &     \SIRFA &            IRNN &         \SEIRNN &          \SIRFA &            IRNN &    \SEIRNN &          \SIRFA &            IRNN &     \SEIRNN &          \SIRFA &            IRNN &     \SEIRNN &      \SIRFA \\
\midrule
7       &  Skill &            0.74 &  \bf{0.76} &       0.68 &            0.60 &  \bf{0.61} &            0.56 &  \bf{0.51} &       0.42 &            0.35 &  \bf{0.61} &        0.52 &            0.51 &  \bf{0.61} &        0.56 &        0.51 \\
     &    MAE &            0.25 &  \bf{0.20} &       0.22 &            0.32 &  \bf{0.31} &  \bf{0.31} &  \bf{0.36} &       0.58 &            0.60 &  \bf{0.28} &        0.32 &            0.34 &  \bf{0.30} &        0.35 &        0.37 \\
     &   $r$ &            0.86 &  \bf{0.92} &       0.89 &  \bf{0.93} &            0.92 &            0.91 &  \bf{0.98} &       0.96 &            0.94 &  \bf{0.93} &        0.89 &            0.90 &  \bf{0.93} &        0.92 &        0.91 \\
\midrule
14      &  Skill &  \bf{0.69} &            0.60 &       0.56 &  \bf{0.53} &            0.47 &            0.46 &  \bf{0.43} &       0.31 &            0.26 &  \bf{0.58} &        0.38 &            0.41 &  \bf{0.55} &        0.43 &        0.41 \\
     &    MAE &  \bf{0.28} &            0.30 &       0.35 &  \bf{0.38} &            0.45 &            0.44 &  \bf{0.44} &       0.76 &            0.77 &  \bf{0.31} &        0.45 &            0.46 &  \bf{0.35} &        0.49 &        0.51 \\
     &   $r$ &            0.79 &  \bf{0.82} &       0.77 &  \bf{0.90} &            0.83 &            0.82 &  \bf{0.97} &       0.90 &            0.90 &  \bf{0.90} &        0.76 &            0.78 &  \bf{0.89} &        0.83 &        0.82 \\
\midrule
21      &  Skill &  \bf{0.60} &            0.49 &       0.47 &  \bf{0.43} &            0.40 &            0.41 &  \bf{0.37} &       0.24 &            0.23 &  \bf{0.51} &        0.31 &            0.35 &  \bf{0.47} &        0.35 &        0.35 \\
     &    MAE &  \bf{0.35} &            0.37 &       0.41 &  \bf{0.50} &            0.54 &            0.51 &  \bf{0.64} &       0.92 &            0.91 &  \bf{0.42} &        0.52 &            0.50 &  \bf{0.48} &        0.59 &        0.58 \\
     &   $r$ &  \bf{0.71} &            0.70 &       0.64 &  \bf{0.80} &            0.76 &            0.76 &  \bf{0.92} &       0.85 &            0.89 &  \bf{0.82} &        0.66 &            0.71 &  \bf{0.81} &        0.74 &        0.75 \\
\midrule
28      &  Skill &  \bf{0.49} &            0.42 &       0.40 &  \bf{0.39} &            0.37 &  \bf{0.39} &            0.21 &       0.21 &  \bf{0.23} &  \bf{0.48} &        0.29 &            0.33 &  \bf{0.37} &        0.31 &        0.33 \\
     &    MAE &            0.51 &  \bf{0.43} &       0.51 &            0.57 &            0.56 &  \bf{0.51} &  \bf{0.86} &       1.09 &            0.99 &            0.50 &        0.55 &  \bf{0.48} &  \bf{0.61} &        0.66 &        0.62 \\
     &   $r$ &  \bf{0.69} &            0.56 &       0.50 &            0.74 &            0.77 &  \bf{0.78} &            0.90 &       0.80 &  \bf{0.91} &  \bf{0.79} &        0.65 &            0.71 &  \bf{0.78} &        0.70 &        0.73 \\
\bottomrule
\end{tabular}


==> Tables/Chapter_2/N_ODE_Results.tex <==
\begin{tabular}{p{1.2cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}p{1.0cm}}
\ $\gamma$ & Metric  &\multicolumn{3}{c}{2015/16} & \multicolumn{3}{c}{2016/17} & \multicolumn{3}{c}{2017/18} & \multicolumn{3}{c}{2018/19} & \multicolumn{3}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}\cmidrule(lr){12-14}\cmidrule(lr){15-17}
   &     &              Fa &              Fp &            FaFp &              Fa &              Fp &            FaFp &              Fa &         Fp &            FaFp &              Fa &          Fp &            FaFp &              Fa &          Fp &            FaFp \\
\midrule
7  &  Skill &            0.82 &            0.81 &  \textbf{0.84} &            0.72 &            0.74 &  \textbf{0.81} &            0.57 &       0.50 &  \textbf{0.66} &            0.63 &        0.66 &  \textbf{0.70} &            0.68 &        0.66 &  \textbf{0.75} \\
   &    MAE &            0.20 &            0.20 &  \textbf{0.19} &            0.28 &            0.25 &  \textbf{0.22} &            0.34 &       0.44 &  \textbf{0.26} &            0.29 &        0.27 &  \textbf{0.26} &            0.28 &        0.29 &  \textbf{0.23} \\
   &   $r$ &  \textbf{0.92} &            0.92 &            0.92 &            0.95 &            0.95 &  \textbf{0.96} &            0.98 &       0.97 &  \textbf{0.99} &            0.94 &        0.94 &  \textbf{0.96} &            0.95 &        0.95 &  \textbf{0.96} \\
\midrule
14 &  Skill &            0.60 &            0.61 &  \textbf{0.68} &            0.53 &            0.51 &  \textbf{0.63} &            0.34 &       0.34 &  \textbf{0.38} &  \textbf{0.47} &        0.41 &            0.41 &            0.47 &        0.46 &  \textbf{0.51} \\
   &    MAE &            0.32 &  \textbf{0.29} &            0.29 &            0.42 &            0.36 &  \textbf{0.32} &            0.59 &       0.71 &  \textbf{0.47} &            0.42 &        0.48 &  \textbf{0.40} &            0.44 &        0.46 &  \textbf{0.37} \\
   &   $r$ &  \textbf{0.84} &            0.84 &            0.84 &            0.87 &            0.89 &  \textbf{0.92} &            0.92 &       0.89 &  \textbf{0.94} &            0.85 &        0.83 &  \textbf{0.87} &            0.87 &        0.86 &  \textbf{0.89} \\
\midrule
21 &  Skill &            0.48 &            0.48 &  \textbf{0.61} &            0.44 &            0.41 &  \textbf{0.54} &  \textbf{0.27} &       0.27 &            0.25 &  \textbf{0.38} &        0.32 &            0.28 &            0.38 &        0.36 &  \textbf{0.39} \\
   &    MAE &            0.39 &            0.35 &  \textbf{0.32} &            0.49 &  \textbf{0.43} &            0.44 &            0.79 &       0.90 &  \textbf{0.75} &  \textbf{0.49} &        0.56 &            0.54 &            0.54 &        0.56 &  \textbf{0.51} \\
   &   $r$ &            0.75 &            0.74 &  \textbf{0.80} &            0.82 &  \textbf{0.85} &            0.84 &  \textbf{0.86} &       0.81 &            0.84 &  \textbf{0.78} &        0.76 &            0.77 &            0.80 &        0.79 &  \textbf{0.81} \\
\midrule
28 &  Skill &            0.42 &            0.42 &  \textbf{0.47} &  \textbf{0.42} &            0.38 &            0.38 &  \textbf{0.24} &       0.23 &            0.17 &  \textbf{0.35} &        0.30 &            0.19 &  \textbf{0.35} &        0.32 &            0.27 \\
   &    MAE &            0.48 &  \textbf{0.37} &            0.43 &  \textbf{0.46} &            0.46 &            0.55 &  \textbf{0.96} &       1.11 &            1.04 &  \textbf{0.51} &        0.58 &            0.70 &  \textbf{0.60} &        0.63 &            0.68 \\
   &   $r$ &            0.64 &            0.66 &  \textbf{0.72} &            0.82 &  \textbf{0.86} &            0.77 &  \textbf{0.84} &       0.76 &            0.71 &  \textbf{0.76} &        0.76 &            0.61 &  \textbf{0.77} &        0.76 &            0.70 \\
\bottomrule
\end{tabular}


==> Tables/Chapter_2/dante_comparison.tex <==
\begin{tabular}{p{0.6cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}}
\ Horizon & Metric  &\multicolumn{5}{c}{2015/16} & \multicolumn{5}{c}{2016/17} & \multicolumn{5}{c}{2017/18} & \multicolumn{5}{c}{2018/19} & \multicolumn{5}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-8}\cmidrule(lr){9-14}\cmidrule(lr){15-20}\cmidrule(lr){16-21}\cmidrule(lr){22-27}
$\gamma$   &     &     Dte &            IRNN &             \FA &         \SEIRNN &     \SIRFA &             Dte &       IRNN &             \FA &     \SEIRNN &      \SIRFA &   Dante &            IRNN &             \FA &     \SEIRNN &          \SIRFA &             Dte &            IRNN &         \FA &     \SEIRNN &      \SIRFA &             Dte &              NN &         \FA &     \SEIRNN &      \SIRFA \\
\midrule
7       &  Skill &    0.67 &            0.74 &            0.72 &  \bf{0.76} &       0.68 &            0.63 &       0.60 &  \bf{0.65} &        0.61 &        0.56 &    0.45 &  \bf{0.51} &            0.37 &        0.42 &            0.35 &  \bf{0.62} &            0.61 &        0.59 &        0.52 &        0.51 &            0.59 &  \bf{0.61} &        0.56 &        0.56 &        0.51 \\
     &    MAE &    0.22 &            0.25 &            0.24 &  \bf{0.20} &       0.22 &  \bf{0.19} &       0.32 &            0.30 &        0.31 &        0.31 &    0.39 &  \bf{0.36} &            0.72 &        0.58 &            0.60 &  \bf{0.21} &            0.28 &        0.29 &        0.32 &        0.34 &  \bf{0.25} &            0.30 &        0.39 &        0.35 &        0.37 \\
     &   $r$ &    0.88 &            0.86 &            0.90 &  \bf{0.92} &       0.89 &  \bf{0.96} &       0.93 &            0.94 &        0.92 &        0.91 &    0.97 &  \bf{0.98} &            0.96 &        0.96 &            0.94 &  \bf{0.97} &            0.93 &        0.93 &        0.89 &        0.90 &  \bf{0.95} &            0.93 &        0.93 &        0.92 &        0.91 \\
\midrule
14      &  Skill &    0.54 &  \bf{0.69} &            0.56 &            0.60 &       0.56 &  \bf{0.54} &       0.53 &            0.50 &        0.47 &        0.46 &    0.29 &  \bf{0.43} &            0.26 &        0.31 &            0.26 &            0.52 &  \bf{0.58} &        0.45 &        0.38 &        0.41 &            0.46 &  \bf{0.55} &        0.43 &        0.43 &        0.41 \\
     &    MAE &    0.38 &  \bf{0.28} &            0.37 &            0.30 &       0.35 &  \bf{0.32} &       0.38 &            0.42 &        0.45 &        0.44 &    0.64 &  \bf{0.44} &            0.86 &        0.76 &            0.77 &            0.33 &  \bf{0.31} &        0.43 &        0.45 &        0.46 &            0.42 &  \bf{0.35} &        0.52 &        0.49 &        0.51 \\
     &   $r$ &    0.64 &            0.79 &  \bf{0.82} &  \bf{0.82} &       0.77 &  \bf{0.91} &       0.90 &            0.85 &        0.83 &        0.82 &    0.90 &  \bf{0.97} &            0.92 &        0.90 &            0.90 &  \bf{0.92} &            0.90 &        0.81 &        0.76 &        0.78 &            0.84 &  \bf{0.89} &        0.85 &        0.83 &        0.82 \\
\midrule
21      &  Skill &    0.44 &  \bf{0.60} &            0.44 &            0.49 &       0.47 &  \bf{0.48} &       0.43 &            0.42 &        0.40 &        0.41 &    0.21 &  \bf{0.37} &            0.20 &        0.24 &            0.23 &            0.46 &  \bf{0.51} &        0.34 &        0.31 &        0.35 &            0.38 &  \bf{0.47} &        0.34 &        0.35 &        0.35 \\
     &    MAE &    0.48 &  \bf{0.35} &            0.47 &            0.37 &       0.41 &  \bf{0.38} &       0.50 &            0.48 &        0.54 &        0.51 &    0.86 &  \bf{0.64} &            0.99 &        0.92 &            0.91 &  \bf{0.40} &            0.42 &        0.53 &        0.52 &        0.50 &            0.53 &  \bf{0.48} &        0.62 &        0.59 &        0.58 \\
     &   $r$ &    0.36 &  \bf{0.71} &  \bf{0.71} &            0.70 &       0.64 &  \bf{0.87} &       0.80 &            0.78 &        0.76 &        0.76 &    0.82 &  \bf{0.92} &            0.90 &        0.85 &            0.89 &  \bf{0.89} &            0.82 &        0.69 &        0.66 &        0.71 &            0.74 &  \bf{0.81} &        0.77 &        0.74 &        0.75 \\
\midrule
28      &  Skill &    0.37 &  \bf{0.49} &            0.38 &            0.42 &       0.40 &  \bf{0.46} &       0.39 &            0.40 &        0.37 &        0.39 &    0.17 &            0.21 &            0.17 &        0.21 &  \bf{0.23} &            0.42 &  \bf{0.48} &        0.27 &        0.29 &        0.33 &            0.33 &  \bf{0.37} &        0.29 &        0.31 &        0.33 \\
     &    MAE &    0.54 &            0.51 &            0.58 &  \bf{0.43} &       0.51 &  \bf{0.39} &       0.57 &            0.47 &        0.56 &        0.51 &    1.06 &  \bf{0.86} &            1.13 &        1.09 &            0.99 &  \bf{0.45} &            0.50 &        0.58 &        0.55 &        0.48 &  \bf{0.61} &  \bf{0.61} &        0.69 &        0.66 &        0.62 \\
     &   $r$ &    0.23 &  \bf{0.69} &            0.58 &            0.56 &       0.50 &  \bf{0.88} &       0.74 &            0.78 &        0.77 &        0.78 &    0.76 &            0.90 &  \bf{0.91} &        0.80 &  \bf{0.91} &  \bf{0.86} &            0.79 &        0.62 &        0.65 &        0.71 &            0.68 &  \bf{0.78} &        0.72 &        0.70 &        0.73 \\
\bottomrule
\end{tabular}


==> Tables/Chapter_2/neuralodecomparison.tex <==
\begin{tabular}{p{1.1cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}}
\ Horizon & Metric  &\multicolumn{4}{c}{2015/16} & \multicolumn{4}{c}{2016/17} & \multicolumn{4}{c}{2017/18} & \multicolumn{4}{c}{2018/19} & \multicolumn{4}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}\cmidrule(lr){19-22}
$\gamma$   &     &     \FA &      \FAQS &  \SIRSIMPLE &     \SIRNN &     \SIRQS &     \SIRFA &    \SEIRNN &    \SEIRFA &     \FA &       \FAQS &  \SIRSIMPLE &      \SIRNN &      \SIRQS &      \SIRFA &     \SEIRNN &     \SEIRFA &     \FA &       \FAQS &  \SIRSIMPLE &      \SIRNN &      \SIRQS &      \SIRFA &     \SEIRNN &     \SEIRFA &     \FA &       \FAQS &  \SIRSIMPLE &      \SIRNN &      \SIRQS &      \SIRFA &     \SEIRNN &     \SEIRFA &     \FA &       \FAQS &  \SIRSIMPLE &      \SIRNN &      \SIRQS &      \SIRFA &     \SEIRNN &     \SEIRFA \\
\midrule
7       &  Skill &    0.72 &       0.90 &        0.58 &       0.64 &       0.42 &       0.68 &       0.76 &       0.75 &    0.65 &        0.66 &        0.45 &        0.56 &        0.36 &        0.56 &        0.61 &        0.63 &    0.37 &        0.53 &        0.19 &        0.33 &        0.06 &        0.35 &        0.42 &        0.39 &    0.59 &        0.63 &        0.23 &        0.50 &        0.27 &        0.51 &        0.52 &        0.57 &    0.56 &        0.67 &        0.32 &        0.50 &        0.23 &        0.51 &        0.56 &        0.57 \\
     &    NLL &    0.20 &      -0.28 &        0.51 &       0.39 &       0.93 &       0.28 &       0.10 &       0.12 &    0.28 &        0.43 &        0.81 &        0.53 &        1.07 &        0.49 &        0.36 &        0.33 &    0.90 &        0.88 &        1.75 &        1.10 &        2.92 &        1.04 &        0.80 &        0.91 &    0.40 &        0.45 &        1.52 &        0.67 &        1.41 &        0.62 &        0.59 &        0.50 &    0.45 &        0.37 &        1.15 &        0.68 &        1.58 &        0.61 &        0.46 &        0.46 \\
     &    MAE &    0.24 &       0.16 &        0.21 &       0.23 &       0.41 &       0.22 &       0.20 &       0.20 &    0.30 &        0.33 &        0.38 &        0.32 &        0.54 &        0.31 &        0.31 &        0.30 &    0.72 &        0.46 &        1.46 &        0.60 &        1.63 &        0.60 &        0.58 &        0.62 &    0.29 &        0.41 &        0.82 &        0.36 &        0.82 &        0.34 &        0.32 &        0.33 &    0.39 &        0.34 &        0.72 &        0.38 &        0.85 &        0.37 &        0.35 &        0.36 \\
     &   CORR &    0.90 &       0.95 &        0.91 &       0.91 &       0.67 &       0.89 &       0.92 &       0.91 &    0.94 &        0.97 &        0.91 &        0.91 &        0.77 &        0.91 &        0.92 &        0.92 &    0.96 &        0.98 &        0.94 &        0.94 &        0.31 &        0.94 &        0.96 &        0.94 &    0.93 &        0.97 &        0.86 &        0.89 &        0.43 &        0.90 &        0.89 &        0.91 &    0.93 &        0.97 &        0.91 &        0.91 &        0.54 &        0.91 &        0.92 &        0.92 \\
\midrule
14      &  Skill &    0.56 &       0.90 &        0.54 &       0.54 &       0.42 &       0.56 &       0.60 &       0.61 &    0.50 &        0.30 &        0.39 &        0.46 &        0.37 &        0.46 &        0.47 &        0.49 &    0.26 &        0.25 &        0.15 &        0.25 &        0.06 &        0.26 &        0.31 &        0.27 &    0.45 &        0.40 &        0.20 &        0.39 &        0.28 &        0.41 &        0.38 &        0.44 &    0.43 &        0.40 &        0.28 &        0.40 &        0.22 &        0.41 &        0.43 &        0.43 \\
     &    NLL &    0.56 &      -0.23 &        0.59 &       0.62 &       0.92 &       0.56 &       0.46 &       0.44 &    0.67 &        2.41 &        0.97 &        0.77 &        1.02 &        0.76 &        0.73 &        0.69 &    1.33 &        2.17 &        1.98 &        1.42 &        3.04 &        1.37 &        1.20 &        1.37 &    0.77 &        1.32 &        1.68 &        0.98 &        1.36 &        0.90 &        0.99 &        0.83 &    0.83 &        1.42 &        1.31 &        0.95 &        1.59 &        0.90 &        0.84 &        0.83 \\
     &    MAE &    0.37 &       0.19 &        0.33 &       0.33 &       0.39 &       0.35 &       0.30 &       0.33 &    0.42 &        0.45 &        0.52 &        0.44 &        0.48 &        0.44 &        0.45 &        0.44 &    0.86 &        0.68 &        1.64 &        0.78 &        1.62 &        0.77 &        0.76 &        0.82 &    0.43 &        0.69 &        0.98 &        0.47 &        0.79 &        0.46 &        0.45 &        0.46 &    0.52 &        0.50 &        0.87 &        0.51 &        0.82 &        0.51 &        0.49 &        0.51 \\
     &   CORR &    0.82 &       0.96 &        0.78 &       0.79 &       0.67 &       0.77 &       0.82 &       0.78 &    0.85 &        0.92 &        0.80 &        0.82 &        0.83 &        0.82 &        0.83 &        0.83 &    0.92 &        0.96 &        0.92 &        0.90 &        0.47 &        0.90 &        0.90 &        0.87 &    0.81 &        0.97 &        0.73 &        0.76 &        0.55 &        0.78 &        0.76 &        0.81 &    0.85 &        0.95 &        0.81 &        0.82 &        0.63 &        0.82 &        0.83 &        0.82 \\
\midrule
21      &  Skill &    0.44 &       0.80 &        0.51 &       0.47 &       0.40 &       0.47 &       0.49 &       0.52 &    0.42 &        0.16 &        0.33 &        0.41 &        0.37 &        0.41 &        0.40 &        0.40 &    0.20 &        0.09 &        0.12 &        0.22 &        0.05 &        0.23 &        0.24 &        0.19 &    0.34 &        0.17 &        0.18 &        0.32 &        0.28 &        0.35 &        0.31 &        0.36 &    0.34 &        0.21 &        0.24 &        0.34 &        0.22 &        0.35 &        0.35 &        0.35 \\
     &    NLL &    0.84 &       0.35 &        0.69 &       0.78 &       0.99 &       0.77 &       0.71 &       0.63 &    0.89 &        5.24 &        1.19 &        0.90 &        1.01 &        0.90 &        0.92 &        0.92 &    1.61 &        6.17 &        2.24 &        1.57 &        3.13 &        1.49 &        1.49 &        1.75 &    1.12 &        2.96 &        1.80 &        1.20 &        1.35 &        1.07 &        1.20 &        1.08 &    1.12 &        3.68 &        1.48 &        1.11 &        1.62 &        1.06 &        1.08 &        1.10 \\
     &    MAE &    0.47 &       0.24 &        0.44 &       0.41 &       0.47 &       0.41 &       0.37 &       0.44 &    0.48 &        0.56 &        0.66 &        0.52 &        0.47 &        0.51 &        0.54 &        0.56 &    0.99 &        0.93 &        1.80 &        0.90 &        1.60 &        0.91 &        0.92 &        1.06 &    0.53 &        1.07 &        1.13 &        0.52 &        0.79 &        0.50 &        0.52 &        0.59 &    0.62 &        0.70 &        1.01 &        0.59 &        0.83 &        0.58 &        0.59 &        0.66 \\
     &   CORR &    0.71 &       0.90 &        0.61 &       0.66 &       0.53 &       0.64 &       0.70 &       0.63 &    0.78 &        0.85 &        0.67 &        0.76 &        0.83 &        0.76 &        0.76 &        0.73 &    0.90 &        0.92 &        0.91 &        0.89 &        0.62 &        0.89 &        0.85 &        0.77 &    0.69 &        0.94 &        0.65 &        0.67 &        0.65 &        0.71 &        0.66 &        0.71 &    0.77 &        0.90 &        0.71 &        0.75 &        0.66 &        0.75 &        0.74 &        0.71 \\
\midrule
28      &  Skill &    0.38 &       0.68 &        0.46 &       0.41 &       0.37 &       0.40 &       0.42 &       0.46 &    0.40 &        0.12 &        0.27 &        0.40 &        0.35 &        0.39 &        0.37 &        0.35 &    0.17 &        0.04 &        0.09 &        0.22 &        0.05 &        0.23 &        0.21 &        0.16 &    0.27 &        0.12 &        0.16 &        0.29 &        0.28 &        0.33 &        0.29 &        0.31 &    0.29 &        0.14 &        0.21 &        0.32 &        0.21 &        0.33 &        0.31 &        0.30 \\
     &    NLL &    1.03 &       1.03 &        0.82 &       0.92 &       1.08 &       0.97 &       0.89 &       0.78 &    0.94 &        7.86 &        1.41 &        0.94 &        1.08 &        0.96 &        1.01 &        1.11 &    1.81 &       14.25 &        2.51 &        1.57 &        3.21 &        1.48 &        1.64 &        1.97 &    1.42 &        3.35 &        1.89 &        1.30 &        1.36 &        1.14 &        1.28 &        1.23 &    1.30 &        6.62 &        1.66 &        1.18 &        1.68 &        1.14 &        1.21 &        1.27 \\
     &    MAE &    0.58 &       0.32 &        0.54 &       0.48 &       0.57 &       0.51 &       0.43 &       0.52 &    0.47 &        0.66 &        0.82 &        0.51 &        0.57 &        0.51 &        0.56 &        0.72 &    1.13 &        1.17 &        1.92 &        1.01 &        1.61 &        0.99 &        1.09 &        1.28 &    0.58 &        1.28 &        1.28 &        0.52 &        0.81 &        0.48 &        0.55 &        0.69 &    0.69 &        0.86 &        1.14 &        0.63 &        0.89 &        0.62 &        0.66 &        0.80 \\
     &   CORR &    0.58 &       0.81 &        0.42 &       0.53 &       0.24 &       0.50 &       0.56 &       0.47 &    0.78 &        0.77 &        0.53 &        0.78 &        0.76 &        0.78 &        0.77 &        0.65 &    0.91 &        0.85 &        0.92 &        0.91 &        0.71 &        0.91 &        0.80 &        0.65 &    0.62 &        0.89 &        0.61 &        0.66 &        0.68 &        0.71 &        0.65 &        0.64 &    0.72 &        0.83 &        0.62 &        0.72 &        0.60 &        0.73 &        0.70 &        0.60 \\
\bottomrule
\end{tabular}


==> Tables/Chapter_2/results_table.tex <==
\begin{tabular}{p{1.1cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}p{0.8cm}}
\ Horizon & Metric  &\multicolumn{4}{c}{2015/16} & \multicolumn{4}{c}{2016/17} & \multicolumn{4}{c}{2017/18} & \multicolumn{4}{c}{2018/19} & \multicolumn{4}{c}{Avg (2015-19)} \\ 
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-14}\cmidrule(lr){15-18}\cmidrule(lr){19-22}
$\gamma$   &     &             \FA &      \SIRSIMPLE &          \SIRNN &          \SIRFA &             \FA &  \SIRSIMPLE &          \SIRNN &          \SIRFA &             \FA &      \SIRSIMPLE &          \SIRNN &          \SIRFA &             \FA &  \SIRSIMPLE &      \SIRNN &          \SIRFA &             \FA &  \SIRSIMPLE &          \SIRNN &          \SIRFA \\
\midrule
7       &  Skill &  \bf{0.72} &            0.58 &            0.64 &            0.68 &  \bf{0.65} &        0.45 &            0.56 &            0.56 &  \bf{0.37} &            0.19 &            0.33 &            0.35 &  \bf{0.59} &        0.23 &        0.50 &            0.51 &  \bf{0.56} &        0.32 &            0.50 &            0.51 \\
     &    NLL &  \bf{0.20} &            0.51 &            0.39 &            0.28 &  \bf{0.28} &        0.81 &            0.53 &            0.49 &  \bf{0.90} &            1.75 &            1.10 &            1.04 &  \bf{0.40} &        1.52 &        0.67 &            0.62 &  \bf{0.45} &        1.15 &            0.68 &            0.61 \\
     &    MAE &            0.24 &  \bf{0.21} &            0.23 &            0.22 &  \bf{0.30} &        0.38 &            0.32 &            0.31 &            0.72 &            1.46 &  \bf{0.60} &  \bf{0.60} &  \bf{0.29} &        0.82 &        0.36 &            0.34 &            0.39 &        0.72 &            0.38 &  \bf{0.37} \\
     &   $r$ &            0.90 &  \bf{0.91} &  \bf{0.91} &            0.89 &  \bf{0.94} &        0.91 &            0.91 &            0.91 &  \bf{0.96} &            0.94 &            0.94 &            0.94 &  \bf{0.93} &        0.86 &        0.89 &            0.90 &  \bf{0.93} &        0.91 &            0.91 &            0.91 \\
\midrule
14      &  Skill &  \bf{0.56} &            0.54 &            0.54 &  \bf{0.56} &  \bf{0.50} &        0.39 &            0.46 &            0.46 &  \bf{0.26} &            0.15 &            0.25 &  \bf{0.26} &  \bf{0.45} &        0.20 &        0.39 &            0.41 &  \bf{0.43} &        0.28 &            0.40 &            0.41 \\
     &    NLL &  \bf{0.56} &            0.59 &            0.62 &  \bf{0.56} &  \bf{0.67} &        0.97 &            0.77 &            0.76 &  \bf{1.33} &            1.98 &            1.42 &            1.37 &  \bf{0.77} &        1.68 &        0.98 &            0.90 &  \bf{0.83} &        1.31 &            0.95 &            0.90 \\
     &    MAE &            0.37 &  \bf{0.33} &  \bf{0.33} &            0.35 &  \bf{0.42} &        0.52 &            0.44 &            0.44 &            0.86 &            1.64 &            0.78 &  \bf{0.77} &  \bf{0.43} &        0.98 &        0.47 &            0.46 &            0.52 &        0.87 &  \bf{0.51} &  \bf{0.51} \\
     &   $r$ &  \bf{0.82} &            0.78 &            0.79 &            0.77 &  \bf{0.85} &        0.80 &            0.82 &            0.82 &  \bf{0.92} &  \bf{0.92} &            0.90 &            0.90 &  \bf{0.81} &        0.73 &        0.76 &            0.78 &  \bf{0.85} &        0.81 &            0.82 &            0.82 \\
\midrule
21      &  Skill &            0.44 &  \bf{0.51} &            0.47 &            0.47 &  \bf{0.42} &        0.33 &            0.41 &            0.41 &            0.20 &            0.12 &            0.22 &  \bf{0.23} &            0.34 &        0.18 &        0.32 &  \bf{0.35} &            0.34 &        0.24 &            0.34 &  \bf{0.35} \\
     &    NLL &            0.84 &  \bf{0.69} &            0.78 &            0.77 &  \bf{0.89} &        1.19 &            0.90 &            0.90 &            1.61 &            2.24 &            1.57 &  \bf{1.49} &            1.12 &        1.80 &        1.20 &  \bf{1.07} &            1.12 &        1.48 &            1.11 &  \bf{1.06} \\
     &    MAE &            0.47 &            0.44 &  \bf{0.41} &  \bf{0.41} &  \bf{0.48} &        0.66 &            0.52 &            0.51 &            0.99 &            1.80 &  \bf{0.90} &            0.91 &            0.53 &        1.13 &        0.52 &  \bf{0.50} &            0.62 &        1.01 &            0.59 &  \bf{0.58} \\
     &   $r$ &  \bf{0.71} &            0.61 &            0.66 &            0.64 &  \bf{0.78} &        0.67 &            0.76 &            0.76 &            0.90 &  \bf{0.91} &            0.89 &            0.89 &            0.69 &        0.65 &        0.67 &  \bf{0.71} &  \bf{0.77} &        0.71 &            0.75 &            0.75 \\
\midrule
28      &  Skill &            0.38 &  \bf{0.46} &            0.41 &            0.40 &  \bf{0.40} &        0.27 &  \bf{0.40} &            0.39 &            0.17 &            0.09 &            0.22 &  \bf{0.23} &            0.27 &        0.16 &        0.29 &  \bf{0.33} &            0.29 &        0.21 &            0.32 &  \bf{0.33} \\
     &    NLL &            1.03 &  \bf{0.82} &            0.92 &            0.97 &  \bf{0.94} &        1.41 &  \bf{0.94} &            0.96 &            1.81 &            2.51 &            1.57 &  \bf{1.48} &            1.42 &        1.89 &        1.30 &  \bf{1.14} &            1.30 &        1.66 &            1.18 &  \bf{1.14} \\
     &    MAE &            0.58 &            0.54 &  \bf{0.48} &            0.51 &  \bf{0.47} &        0.82 &            0.51 &            0.51 &            1.13 &            1.92 &            1.01 &  \bf{0.99} &            0.58 &        1.28 &        0.52 &  \bf{0.48} &            0.69 &        1.14 &            0.63 &  \bf{0.62} \\
     &   $r$ &  \bf{0.58} &            0.42 &            0.53 &            0.50 &  \bf{0.78} &        0.53 &  \bf{0.78} &  \bf{0.78} &            0.91 &  \bf{0.92} &            0.91 &            0.91 &            0.62 &        0.61 &        0.66 &  \bf{0.71} &            0.72 &        0.62 &            0.72 &  \bf{0.73} \\
\bottomrule
\end{tabular}

